Cross-Document Event-Keyed Summarization

Event-keyed summarization (EKS) requires summarizing a specific event described in a document given the document text and an event representation extracted from it. In this work, we extend EKS to the cross-document setting (CDEKS), in which summaries must synthesize information from accounts of the same event as given by multiple sources. We introduce SEAMUS (Summaries of Events Across Multiple Sources), a high-quality dataset for CDEKS based on an expert reannotation of the FAMUS dataset for cross-document argument extraction. We present a suite of baselines on SEAMUS -- covering both smaller, fine-tuned models, as well as zero- and few-shot prompted LLMs -- along with detailed ablations and a human evaluation study, showing SEAMUS to be a valuable benchmark for this new task.

==> sections/04-setup.tex <==
\paragraph{Tasks} We present experiments on both the (single-document) report (\S\ref{sec:experiments::report-summarization}) and cross-document (\S\ref{sec:experiments::cross-doc-summarization}) summarization tasks. In the single-document (EKS) setting, both the report and its annotated event are provided as input. The cross-document setting (CDEKS) is analogous, but augments the input to also include the corresponding source document and its event annotation. In \S\ref{sec:experiments::input-ablations}, we briefly discuss some ablations on the input inspired by similar ones from \citet{gantt-etal-2024-event}, with full results in \autoref{app:additional_results}. Finally, in \S\ref{sec:experiments::extraction-quality}, we consider the impact of degraded argument extraction performance on summarization results.

\paragraph{Models} We benchmark \dataset using models of two types. First, we consider several classic pretrained encoder-decoder models widely used for summarization: BART \citep{lewis-etal-2020-bart}, PEGASUS \citep{zhang-etal-2020-pegasus}, and T5 \citep{raffel-etal-2020-exploring}, fine-tuning the large versions of all three on the \dataset training data. Second, we consider some of the latest proprietary LLMs, evaluated in both the zero- and few-shot settings: GPT-4o\footnote{\tiny{\url{https://openai.com/index/hello-gpt-4o/}}}, GPT-4o mini (\textsc{GPT-4o M} in \autoref{tab:merged-results})\footnote{\tiny{\url{https://openai.com/index/gpt-4o-mini-advancing-cost-efficient-intelligence/}}}, Claude 3 Haiku (\textsc{Claude H})\footnote{\tiny{\url{https://www.anthropic.com/news/claude-3-haiku}}}, and Claude 3.5 Sonnet (\textsc{Claude S})\footnote{\tiny{\url{https://www.anthropic.com/news/claude-3-5-sonnet}}}. For the few-shot examples, we use the three examples from the train split whose frame matches that of the target example. Finally, we also report a naïve ``report baseline'' (\textsc{RB}) that treats the report text itself as the predicted summary.


\paragraph{Metrics} We report several standard summarization metrics, including ROUGE-1 ($\textbf{R}_1$), ROUGE-2 ($\textbf{R}_2$), and ROUGE-LCS $\text{F}_1$ scores \citep[$\textbf{R}_L$;][]{lin-2004-rouge}, and BERTScore $\text{F}_1$ \citep[\textbf{BS};][]{zhang-etal-2019-bertscore}.

Given our focus on producing summaries that recover \emph{specific} pieces of information---as captured by an event's roles---we report several other metrics that evaluate this. First, we report CEAF-REE \citep[\textbf{CR};][]{du-etal-2021-grit}, a form of argument $\text{F}_1$ that allows us to compare arguments extracted from a \emph{predicted} summary against those in a \emph{reference} summary, aligning arguments based on exact match.\footnote{We also provide results with a soft-match variant of this metric in \autoref{app:additional_results}} We train the event extraction model of \citet{xia-etal-2021-lome} on \dataset and use it to extract arguments from the predicted summaries, constraining extraction to arguments satisfying licit roles of the target frame.

The summaries in \dataset naturally also make claims about these arguments. To evaluate these claims' faithfulness to the text, we report AlignScore \citep[\textbf{A};][]{zha-etal-2023-alignscore}, a learned metric that provides a unit score that indicates how well a \emph{claim} (here, a summary) is supported by a \emph{context} (the report text for the report-only task, and the concatenated report and source texts for the combined task).

% FActScore \citep[\textbf{F};][]{min-etal-2023-factscore}, which decomposes each summary into a set of atomic facts and reports the average \% of these that are supported by a given knowledge source (here, the concatenated report and source texts).

% and CEAF-REE \citep{du-etal-2021-grit}. \citet{gantt-etal-2024-event} additionally report a suite of NLI-based metrics, introduced by \citet{chen-eger-2023-menli}, which compute entailment probabilities---using the predicted summary as the hypothesis and either the document or the reference summary as the premise. However, a growing body of work casts doubt on the effectiveness of such metrics, owing to the large distributional shift between the overwhelmingly sentence-level NLI datasets used to train them and the document-level texts of summarization tasks \citep[][\emph{i.a.}]{laban-etal-2022-summac, zha-etal-2023-alignscore}.
